Nearly Optimal Resource Allocation for Downlink OFDMA in 2-D Cellular Networks

In this paper, we propose a resource allocation algorithm for the downlink of sectorized two-dimensional (2-D) OFDMA cellular networks assuming statistical Channel State Information (CSI) and fractional frequency reuse. The proposed algorithm can be implemented in a distributed fashion without the need to any central controlling units. Its performance is analyzed assuming fast fading Rayleigh channels and Gaussian distributed multicell interference. We show that the transmit power of this simple algorithm tends, as the number of users grows to infinity, to the same limit as the minimal power required to satisfy all users' rate requirements i.e., the proposed resource allocation algorithm is asymptotically optimal. As a byproduct of this asymptotic analysis, we characterize a relevant value of the reuse factor that only depends on an average state of the network.

==> commandes.tex <==
% Packages


% Theoremes
\newtheorem{remark}{Remark}
\newtheorem{prop}{Proposition}
\newtheorem{result}{Result}
\newtheorem{problem}{Problem}
\newtheorem{theo}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{conj}{Conjecture}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{corollary}{Corollary}


% Titres
\newcommand{\Headingtitre}[1]{\begin{center}\Large\bf\sc #1\end{center}}
\newcommand{\headingtitre}[1]{\begin{center}\large\bf\sc #1\end{center}}
\newcommand{\heading}[1]{\begin{center}\large \underline{#1}\end{center}}
\newcommand{\headingmf}[1]{\large\bf\it \underline{#1}}
\newcommand{\titre}[1]{\begin{center}\large\it {#1}\end{center}}


% Couleurs
\usepackage{color}
\definecolor{MyDarkBlue}{rgb}{0.1,0,0.65}
\definecolor{MyDarkRed}{rgb}{.85,0,0.1}

% Symboles 
\newcommand{\tr}[1]{\textrm{tr}\left(#1\right)}
\newcommand{\tri}{$\triangleright$}
\newcommand{\btri}{{\color{MyDarkBlue} $\triangleright$}}
\newcommand{\bbul}{{\color{MyDarkBlue} $\bullet$}}

% Espacement
\newcommand{\RR}{\vspace*{.2cm}\\}


% Macro math g\'en\'erales
\newcommand{\real}[1]{{\mathfrak{R}}\left[#1\right]}
\newcommand{\imag}[1]{{\mathfrak{I}}\left[#1\right]}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\diag}[1]{\textrm{diag}\left(#1\right)}
\newcommand{\trace}[1]{\textrm{Trace}\left(#1\right)}
\newcommand{\card}[1]{\textrm{card}\left(#1\right)}
\newcommand{\EE}[1]{{\mathbb{E}}\left[ #1 \right]}
\newcommand{\PP}[1]{{\mathbb{P}}\left\{ #1 \right\}}
\newcommand{\Pout}{{\mathbb{P}}_\textrm{out}}
\newcommand{\oo}{\textrm{o}}
\newcommand{\ud}{\textrm{d}}
\renewcommand{\i}{\imath}
%\renewcommand{\QED}{\QEDopen}
\providecommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\bs}{\boldsymbol}
\newcommand{\dsp}{\displaystyle}
\newcommand{\dron}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ddron}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\dddron}[3]{\frac{\partial^2 #1}{\partial #2 \:\partial #3}}

% Macro synchro
\newcommand{\df}{\delta\! f}
\newcommand{\dfk}{\delta\! f_k}
\newcommand{\ok}{\omega_k}
\newcommand{\CRBN}{\overline{CRB}_N}
\newcommand{\Nk}{_{N,k}}
\newcommand{\Nl}{_{N,l}}

% Macro relay
\newcommand{\Pc}{P_{\cal C}}
\newcommand{\Pco}{P_{{\cal C}_0}}
%\newcommand{\Tc}{{\cal T}_{\cal C}}
\newcommand{\Tco}{{\cal T}_{{\cal C}_0}}
\newcommand{\Sc}{{\cal S}_{\cal C}}
\newcommand{\Sco}{{\cal S}_{{\cal C}_0}}
\newcommand{\bx}{{\bf x}}
\newcommand{\by}{{\bf y}}
\newcommand{\bX}{{\bf X}}
\newcommand{\bY}{{\bf Y}}
\newcommand{\bXoo}{{\bf X}_{00}}
\newcommand{\bXou}{{\bf X}_{01}}
\newcommand{\bYuo}{{\bf Y}_{10}}
\newcommand{\bXuu}{{\bf X}_{11}}
\newcommand{\bYdo}{{\bf Y}_{20}}
\newcommand{\bYdu}{{\bf Y}_{21}}

% Macro Nassar
\newcommand{\ki}{_{k,i}}
\newcommand{\ku}{_{k,1}}
\newcommand{\kd}{_{k,2}}
\newcommand{\li}{_{l,i}}
\newcommand{\lu}{_{l,1}}
\newcommand{\ld}{_{l,2}}
\newcommand{\Lu}{_{L,1}}
\newcommand{\Lpu}{_{L+1,1}}
\newcommand{\Ld}{_{L,2}}
\newcommand{\Lpd}{_{L+1,2}}
\newcommand{\Lp}{_{L+1}}
\newcommand{\A}{{\cal A}}
\newcommand{\Au}{{\cal A}_1}
\newcommand{\Ad}{{\cal A}_2}
\newcommand{\Ai}{{\cal A}_i}
\newcommand{\K}{^{(K)}}
\newcommand{\cK}{^{c,(K)}}
\newcommand{\cpK}{^{c,(\phi_K)}}
\newcommand{\ctK}{^{c,(\theta_K)}}
\newcommand{\cpsiK}{^{c,(\psi_K)}}
\newcommand{\ApK}{^{A,(\phi_K)}}
\newcommand{\BpK}{^{B,(\phi_K)}}
\newcommand{\AK}{^{A,(K)}}
\newcommand{\BK}{^{B,(K)}}
\newcommand{\cbarK}{^{\overline{c},(K)}}
\newcommand{\QujA}{Q_{1,j}^A}
\newcommand{\QujB}{Q_{1,j}^B}
\newcommand{\QdjA}{Q_{2,j}^A}
\newcommand{\QdjB}{Q_{2,j}^B}
\newcommand{\QjA}{Q_{j}^A}
\newcommand{\QjB}{Q_{j}^B}
\newcommand{\QdiA}{Q_{2,\infty}^A}
\newcommand{\QdiB}{Q_{2,\infty}^B}
\newcommand{\QuiA}{Q_{1,\infty}^A}
\newcommand{\QuiB}{Q_{1,\infty}^B}
\newcommand{\QiA}{Q_{\infty}^A}
\newcommand{\QiB}{Q_{\infty}^B}
